Double InfoGAN for Contrastive Analysis

Contrastive Analysis (CA) deals with the discovery of what is common and what is distinctive of a target domain compared to a background one. This is of great interest in many applications, such as medical imaging. Current state-of-the-art (SOTA) methods are latent variable models based on VAE (CA-VAEs). However, they all either ignore important constraints or they don't enforce fundamental assumptions. This may lead to sub-optimal solutions where distinctive factors are mistaken for common ones (or viceversa). Furthermore, the generated images have a rather poor quality, typical of VAEs, decreasing their interpretability and usefulness. Here, we propose Double InfoGAN, the first GAN based method for CA that leverages the high-quality synthesis of GAN and the separation power of InfoGAN. Experimental results on four visual datasets, from simple synthetic examples to complex medical images, show that the proposed method outperforms SOTA CA-VAEs in terms of latent separation and image quality. Datasets and code are available online.

==> supplement_include.tex <==
\begin{center}
    \Large{\textbf{Supplementary Material}}
\end{center}
\section{Ethical Statement}
This paper presents the Double InfoGAN method, which aims to improve the accuracy and interpretability of Contrastive Analysis in various fields, including medical imaging. We acknowledge that the use of medical imaging datasets raises ethical concerns that we discuss in the following. 

Firstly, we ensured that all medical imaging datasets used in our experiments were publicly available, anonimized and ethically sourced. Secondly, we aim at developing a method that improves the quality and interpretability of medical images, potentially leading to better diagnosis and treatment. We recognize that the accuracy and reliability of the generated medical images are crucial for clinical decision-making and that, as already mentioned in the article, more powerful GAN architectures with specific anatomical regularizations will be explored in future. Another ethical concern is the potential for biased outcomes, particularly when the datasets are not representative of the entire population. Biases in the data can lead to inaccurate and unfair results, which could exacerbate healthcare disparities or bring to wrong diagnosis and treatments. Therefore, it is important to ensure that datasets are diverse, inclusive and not biased, representing different demographics, hospitals, conditions, etc. 

In summary, while contrastive analysis can lead to significant improvements in healthcare and in other domains, it is essential to address potential ethical concerns, such as privacy and bias, to ensure accurate and trustworthy results.

\section{Architecture}\label{app:architecture}
We present here the architectures used to obtain the results of this paper. These are inspired by DCGAN \cite{Radford2016}, with the addition of Gaussian Noise in the Discriminator. This prevents it from converging too fast and improves our performances. For the Brats dataset, we also added the spectral norm in the discriminator (instead of the batchnorm), and an attention block in the generator.

All computations are run on a server with one NVIDIA A100 GPU card and 64 AMD EPYC 7302 16-Core Processors.

\begin{table}[h!]
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l| l |}
\hline
Discriminator D / C / Q & Generator G \\
\hline
Input $64\times 64 \times c $ ; c=3 for RGB, c=1 for gray/binary & Input  $ z \in \mathbb{R}^n, s \in \mathbb{R}^m $ \\

Gaussian noise, $4\times4$ conv 64, stride 2, lReLU & concat and reshape $(z+s,1,1)$ \\
Gaussian noise, $4\times4$ conv 128, stride 2, batchnorm, lReLU & $4 \times 4$ convtranspose 512, batchnorm, ReLU \\
Gaussian noise, $4\times4$ conv 256, stride 2, batchnorm, lReLU & $4 \times 4$ convtranspose 256, stride 2, batchnorm, ReLU  \\
Gaussian noise, $4\times4$ conv 512, stride 2, batchnorm, lReLU (*) & $4 \times 4$ convtranspose 128, stride 2, batchnorm, ReLU  \\
From *:  Gaussian noise, $4\times4$ conv 1, sigmoid (output layer for D) & $4 \times 4$ convtranspose 64, stride 2, batchnorm, ReLU  \\
From *:  Gaussian noise, $4\times4$ conv 1, sigmoid (output layer for C) &  $4 \times 4$ convtranspose c , stride 2, Tanh  \\
From *: Gaussian noise, $4\times4$ conv n (output layer for $Q_z$) & \\
From *: Gaussian noise, $4\times4$ conv m (output layer for $Q_s$) & \\
\hline
\end{tabular}
\end{adjustbox}
\end{center}
\caption{Architecture for celeba, cifar/mnist and dsprite/mnist datasets. Gaussian Noise is added at every layer, with standard deviation of 0.2. LeakyReLU has a negative slope of 0.2. Batch size of 128. When a CR module is added, it has the same architecture as $Q_s$}
\end{table}


\begin{table}[h!]
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l| l |}
\hline
Discriminator D / C / Q & Generator G \\
\hline
Input $128\times 128 \times 1 $ & Input  $ z \in \mathbb{R}^n, s \in \mathbb{R}^m $ \\

Gaussian noise, $4\times4$ conv 64, stride 2, spectral norm, lReLU & concat + FC $8192$ +reshape $(512,4,4)$ \\
Gaussian noise, $4\times4$ conv 128, stride 2, spectral norm, lReLU & upsample, $3 \times 3$ conv 1024, batchnorm, ReLU \\
Gaussian noise, $4\times4$ conv 256, stride 2, spectral norm, lReLU &  upsample, $3 \times 3$ conv 512, batchnorm, ReLU  \\
Gaussian noise, $4\times4$ conv 512, stride 2, spectral norm, lReLU &  upsample, $3 \times 3$ conv 256, batchnorm, ReLU \\
Gaussian noise, $4\times4$ conv 512, stride 2, spectral norm, lReLU (*) & Self-Attention Block  \\
From *:  Gaussian noise, FC $1$, sigmoid (output layer for D) &upsample, $3 \times 3$ conv 256, batchnorm, ReLU  \\
From *:  Gaussian noise, FC 1, sigmoid (output layer for C) & $3 \times 3$ conv 128, batchnorm, ReLU \\
From *: Gaussian noise, FC 128 , spectral norm, lReLU &  upsample, $3 \times 3$ conv 64, batchnorm, ReLU  \\
Gaussian noise, FC n , spectral norm, lReLU (output layer for $Q_z$) &  $3 \times 3$ conv 1, tanh \\
From *: Gaussian noise , FC 128 , SN, lReLU & \\
Gaussian noise, FC m , spectral norm, lReLU (output layer for $Q_s$) & \\
\hline
\end{tabular}
\end{adjustbox}
\end{center}
\caption{Architecture for Brats. Gaussian noise is additive, with standard deviation of 0.2. LeakyReLU has a negative slope of 0.2. Batch size of 32.}
\end{table}
\newpage

\section{Mathematical developments}\label{app:math}
\subsection{InfoGAN and InfoGAN-CR}\label{app:InfoGAN}
The regularization loss proposed in InfoGAN \cite{chen_infogan_2016} is:


\begin{equation}
\begin{split}
 &I(\bc;\bx) = -H(\bc|\bx) + H(\bc) = \bbE_{\bx \sim P(\bx), \bc \sim P(\bc|\bx)} \log P(\bc|\bx) + H(\bc)= \\
 &=\int P(\bx) \int P(\bc|\bx)  \log(P(\bc|\bx)) dx dc + H(\bc) =\\
&=\int P(\bx) \int P(\bc'|\bx)  \log(P(\bc'|\bx)) dx dc' + H(\bc') = \quad \text{(change of variables between c and c')}\\
&=\int \int \int P(\bx, \bc, \bz) dc dz \int P(\bc'|\bx)  \log(P(\bc'|\bx)) dx dc' + H(\bc') =\\
&=\int P(\bz) \int P(\bc) \int P(\bx|\bc, \bz) \int P(\bc'|\bx)  \log(P(\bc'|\bx)) dz dx dc' dc + H(\bc') =\\
&=\int P(\bz) \int P(\bc) \int P(\bx|\bc, \bz) \int P(\bc'|\bx)  \log(P(\bc'|\bx) \frac{Q(\bc'|\bx)}{Q(\bc'|\bx)}) dz dx dc' dc + H(\bc') = \quad \text{(identity trick)}\\
 &= \underbrace{\bbE_{\bz \sim P(\bz), \bc \sim P(\bc),\bx \sim P(\bx |\bc, \bz)} KL(P(\bc'|\bx) || Q(\bc'|\bx))}_{\geq 0} + \bbE_{\bz \sim P(\bz), \bc \sim P(\bc),\bx \sim P(\bx |\bc, \bz)} \bbE_{c' \sim P(\bc'|\bx)} \log Q(\bc'|\bx) + H(\bc')\\
 &\geq  \bbE_{\bz \sim P(\bz), \bc \sim P(\bc),\bx \sim P(\bx |\bc, \bz)} \bbE_{\bc' \sim P(\bc'|\bx)} \log( Q(\bc'|\bx)) + H(\bc')
 \label{app:InfoGAN-I}
\end{split}
\end{equation}

where we have introduced an auxiliary distribution $Q(\bc|\bx)$, parameterized as a neural network, to approximate the posterior $P(\bc|\bx)$ (which is difficult to compute) and we have made the hypothesis that $\bc$ does not depend on $\bz$ (i.e., $P(\bc|\bz)=P(\bc)$). To further remove also the need to sample from $P(\bc|\bx)$ (which would be impossible in most cases), authors propose a simple, yet effective, modification of the previous variational lower bound. In their algorithm, they actually compute and maximize: $\cL(G,Q) = \bbE_{\bz \sim P(\bz), \bc \sim P(\bc),x \sim P(\bx |\bc, \bz)} \log(Q(\bc|\bx)) + H(\bc)$, which is equivalent to the previous lower bound:

\begin{equation}
\begin{split}
&\cL(G,Q) = \bbE_{\bz \sim P(\bz), \bc \sim P(\bc),\bx \sim P(\bx |\bc, \bz)} \log(Q(\bc|\bx)) + H(\bc)=\\
&= \int P(\bz) \int P(\bc) \int P(\bx |\bc,\bz) \log(Q(\bc|\bx)) dz dc dx + H(\bc)=\\
&= \int P(\bz) \int \int  P(\bx, \bc|\bz) \log(Q(\bc|\bx)) dz dc dx + H(\bc)=\\
&= \int P(\bz) \int \int  P(\bx, \bc'|\bz) \log(Q(\bc'|\bx)) dz dc' dx + H(\bc')= \quad \text{(change of variable between c and c')}\\
&=\int P(\bz) \int \int  P(\bx | \bz) P(\bc'|\bx,\bz)  \log(Q(\bc'|\bx)) dz dc' dx + H(\bc')=\\ 
&=\int P(\bz) \int \int \int P(\bx, \bc | \bz) P(\bc'|\bx)  \log(Q(\bc'|\bx)) dz dc' dx dc + H(\bc') = \quad \text{(c' does not depend on z and re-introduce c)}\\
&=\int P(\bz) \int \int \int P(\bc) P(\bx |\bc, \bz) P(\bc'|\bx)  \log(Q(\bc'|\bx)) dz dc' dx dc + H(\bc') =\\
 &= \bbE_{\bz \sim P(\bz), \bc \sim P(\bc),\bx \sim P(\bx |\bc, \bz)} \bbE_{\bc' \sim P(\bc'|\bx)} \log(Q(\bc'|\bx)) + H(\bc')
 \label{app:InfoGAN-loss}
\end{split}
\end{equation}

In \cite{chen_infogan_2016}, authors proposed to model the auxiliary conditional distribution $Q(\bc|\bx)$ as a \textit{factorized Gaussian} with \textit{identity covariance} $Q(\bc|\bx) = 
 \prod_i (c_i|\bx) = \prod_i  \cN(\mu_i(\bx), 1)$. As shown in \cite{Lin2020}, this is fundamental for stability and efficiency. Furthermore, in \cite{Lin2020}, authors also showed that informativeness alone does not necessarily encourage disentanglement. To this end, they propose a new regularizer, called \textit{Contrastive Regularizer} (CR), which enforces distinguishable visual changes in the images created using different latent codes. More specifically, they propose to fix a latent code $c_i$, draw the others $\{ c_j \}_{j \neq i}$ uniformly at random, and then sample two or more images $x_i$ from the resulting distribution $(x_i) \sim Q^i$. By repeating this process for all $k$ latent codes $c_i$, one can obtain an estimate of all distributions $Q^i$. The goal, following the usual definition of disentanglement, is then to maximize the difference between the distributions $Q^i$, so that each latent code $c_i$ should encode a specific visual variation in the created images that should be noticeable and easy to distinguish from the patterns encoded by the other latent codes $\{ c_j \}_{j \neq i}$. 
 Authors propose to maximize the following loss:

 \begin{equation}
  \cL_c = d_{JS}(Q^1,...,Q^k) := \frac{1}{k} \sum_i KL(Q^i || \frac{\sum_{j} Q^j}{k})   
 \end{equation}

They propose to approximate this regularization term using a discriminator $H$ that performs multi-way hypothesis testing. Given two or more images $(x_i)$, created by fixing only one latent code $c_i$, the discriminator $H$ needs to identify the latent dimension $i$ shared between the images. Authors claim, and experimentally demonstrate, that by updating both discriminator $H$ and generator $G$ to maximize $\cL_c$ it "should encourage each latent code $c_i$ to make distinct and noticeable changes, hence promoting disentanglement". 

We adapted the CR module for our model, as explained in Fig.\ref{fig:cr}.


% \begin{figure}[h]
% 	\begin{center}
%     \centering
%     \resizebox{0.9\textwidth}{!}{%
% 	\begin{tikzpicture}[node distance=1cm, auto,]
	
% 	\node[rectangle,
%     draw = black,
%     text = black,
%     minimum width = 0.5cm, 
%     minimum height = 0.5cm] (c) at (-7.2,0.7) {\large $z \in \bbR^L$}; 

%     %\node[rectangle,
%     %draw = black,
%     %text = black,
%     %minimum width = 1.7cmcm, 
%     %text width = 2.8cm,
%     %minimum height = 0.6cm] (n) at (-11.2,-0.7) {\large sample $k \in \mathbb{N}$, $k < m $}; 

%     \node[rectangle,
%     draw = black,
%     text = black,
%     minimum width = 1.0cm,
%     text width = 3.1cm,
%     minimum height = 0.6cm] (n) at (-7.4,-0.7) {\large  $s^1, s^2 \in \bbR^M$, \\  $s^{1}_k = s^2_k \\ s^{1}_j \neq s^2_j \quad \forall j \neq k$};
    
%     %\draw [line width=0.5pt] [->]  (-9.6,-0.7) -- (-9.1,-0.7);
    
% 	\draw [line width=0.5pt] [-]  (-5.0,-0.5) -- (-5.0,0.5) --(-3.5,1.0) -- (-3.5,-1.0) -- (-5.0,-0.5);
% 	\node (g) at (-4.2,0){\large$G$};

%     \draw [line width=0.5pt] [->]  (-5.7,0.7) -- (-5.1,0.1);
%     \draw [line width=0.5pt] [->]  (-5.7,-0.7) -- (-5.1,-0.1);
    
%     \node[rectangle,
%     draw = black,
%     text = black,
%     minimum width = 2.4cm, 
%     minimum height = 1.5cm] (r) at (-2.0,1.0) {\large $G(z,s^1)$};

%       \node[rectangle,
%     draw = black,
%     text = black,
%     minimum width = 2.4cm, 
%     align = center,
%     minimum height = 1.5cm] (r) at (-2.0,-0.9) {\large $G(z,s^2)$};


%     %\node[rectangle,
%     %draw = black,
%     %text = black,
%     %minimum width = 2.4cm, 
%     %align = center,
%     %minimum height = 1.5cm] (r) at (1.0,0.0) {concat};
%     %\draw [line width = 0.5pt] [-] (0.0,0.75) -- (0.0,1.0) -- (2.4,1.0) -- (2.4,-0.5) -- (2.2,-0.5) ;
    
%     \draw [line width=0.5pt] [->]  (-0.6,1.0) -- (-0.1,0.5);
%     \draw [line width=0.5pt] [->]  (-0.6,-1) -- (-0.1,-0.5);
    
    
% 	\draw [line width=0.5pt] [-]  (0,-1) -- (0,1) --(1.5,0.5) -- (1.5,-0.5) -- (0,-1);
% 	\node (d) at (0.8,0){\large $H$};

%     \node (k2) at (3.0,0) {$\begin{matrix} 0 \\ 1 \\ \vdots \\ k \\ \vdots \end{matrix} $ $\begin{bmatrix} 0.02 \\ 0.06 \\ \vdots \\ 0.7 \\ \vdots \end{bmatrix}$};

%     \draw [line width=0.5pt] [->]  (1.6,0) -- (2.1,0);

    
		
% 	\end{tikzpicture}
% 	}
% 	\end{center}
\begin{figure}[h]
    \centering
\includegraphics[width=14cm]{figures/ContrastiveReg.png}
\caption{Contrastive regularizer. Two images are generated with the following constraints: the background latent space $z$ is the same, and all the salient latent code are different except one (named $k$ here). From these two images, the CR module is then trained to predict which one of the latent code was identical. The CR module outputs a vector of probabilities of the same size as $s$.}
    \label{fig:cr}
\end{figure}

%\PG{IDEA: if all latent codes are between (-3 and +3), one could also fix all latent codes $\{ c_j \}_{j \neq i}$ to a certain value, and then sample the remaining latent code $c_i$ uniformly between -3 and +3. Then, the discriminator $H$, or another one, should also predict the good order. Or, given image at -1 and +1 it should be able to predict image at 0. Or, given many images created with different codes, it should correctly find the image coming from the same latent code.}


%\subsection{Contrastive VAE} 
%Let $X=\{\bx_i\}_{i=1}^N$ and $Y=\{\by_j\}_{j=1}^M$ be the background (or control) and target data-sets of images respectively. Both $\{\bx_i\}$ and $\{\by_j\}$ are assumed to be i.i.d. from two different  and unknown distributions ($P(\bx)$ and $P(\by)$) that depend on a pair of latent variables ($\bz$, $\bs$). Here, $\bs$ is assumed to capture the salient generative factors proper only to $Y$ whereas $\bz$ should describe the common generative factors between $X$ and $Y$. The generative models are: $\bx_i \sim P_\theta (\bx | \bz_i, \bs_i=s')$ and $\by_j \sim P_\theta (\by_j | \bz_j, \bs_j)$, where the salient factors $\bs_i$ of $X$ are fixed to a constant value $s'$, which is usually assumed to be 0 (i.e., $s'=0$). This implicitly enforces $\bz$ to fully encode alone $X$. Possible factors of variations proper only to $X$, and not to $Y$, are thus discarded from the analysis. Furthermore, the same generative model $P_\theta$ is used for both data-sets. This is usually assumed to follow a Gaussian distribution \cite{zou_joint_2022} parameterized by a neural network (i.e. decoder with parameters $\theta$) or a Laplace distribution \cite{ruiz_learning_2019}. Similarly to standard VAE, the conditional posterior distributions is approximated using another neural network (i.e. encoder with parameters $\phi$) shared between $X$ and $Y$: $Q_\phi(\bz_i,\bs_i|x_i)$ and $Q_\phi(\bz_j,\bs_j|y_j)$. An important assumption always done in the literature is the factorization of $Q_\phi$, namely $Q_\phi(\bz,\bs|\cdot)=Q_\phi(\bz|\cdot)Q_\phi(\bs|\cdot)$. About the latent generative factors ($\bz$, $\bs$), they are usually assumed to be \textit{independent} (i.e., $p_{\cdot}(\bz,\bs)=p_{\cdot}(\bz) p_{\cdot}(\bs)$). The common factor $\bz$ should follow the same distribution in $X$ and $Y$, which is usually defined as an isotropic Gaussian distribution (i.e., $p_{\cdot}(\bz)=\cN(\bz;0,\cI)$). The salient factor $\bs$ follows instead a different prior distribution between $X$ and $Y$ to take into account the different generative models: $P_y(\bs)=\cN(\bs;0,\cI)$ and $P_x(\bs)=\delta(\bs=s')$, where $\delta(\bs=s')$ denotes the Dirac distribution centered at $s'$. Based on this generative latent variable model, one can derive a lower bound of the marginal log likelihood $\log P(\bx)$:
%\begin{equation}
%\begin{split}
%\log P(\bx) \geq & \bbE_{Q_\phi(\bz|\bx)Q_\phi(\bs|\bx)}\log P_\theta(\bx | \bz,\bs)\\
%& - KL(Q_\phi(\bz|\bx) || p_\bx(z))\\
%& - KL(Q_\phi(\bs|\bx) || p_\bx(s))
%\end{split}
%\end{equation}
%and similarly for $\log P(\by)$. 
%SOTA cotrastive VAE methods differ mainly for:\\
%\noindent 1) computation (or not) of the KL divergence term about $p_\by(s)$ (i.e., only \cite{choudhuri_towards_2019} and \cite{weinberger_moment_2022} propose to compute it, all other works simply ignore it). Not computing it can make some information leak between $\bz$ and $\bs$.\\
%\noindent 2) constraining the distribution of $\bz$ to be identical between $X$ and $Y$ (i.e., $Q_\phi(\bz|\bx) \sim Q_\phi(\bz|\by)$), which is only considered in \cite{choudhuri_towards_2019} and \cite{weinberger_moment_2022}.\\
%\noindent 3) adding new losses to the ELBO term such as: loss to actually impose the assumed factorization  of $Q_\phi$ (i.e., $Q_\phi(\bz,\bs|\cdot)=Q_\phi(\bz|\cdot)Q_\phi(\bs|\cdot)$) \cite{abid_contrastive_2019}, adding a classification layer after the encoder to infer the class (background or target) of unlabeled images at test time \cite{zou_joint_2022}, or making symmetric the objective function \cite{ruiz_learning_2019}\\
%\noindent 4) architecture choices (e.g., \cite{zou_joint_2022} uses AdaIn \cite{huang_arbitrary_2017}, \cite{ruiz_learning_2019} uses a $l1$ reconstruction loss). 

\subsection{Double InfoGAN}\label{app:DoubleINFOGAN}
%In Double InfoGAN, we use a generative model similar to the one proposed in Contrastive VAE but within the framework of InfoGAN. Similarly to Contrastive VAE, we suppose that the background images $\{\bx_i\}$ and the target images $\{\by_j\}$ are i.i.d. samples from two different and unknown distributions ($P(\bx)$ and $P(\by)$) that depend on a pair of latent variables ($\bz$, $\bs$). Differently from InfoGAN, $\bz$ should now capture the generative factors common to both $X$ and $Y$ whereas $\bs$ the salient factors proper only to $Y$. Please note that the inclusion of other two factors, similarly to InfoGAN, describing the incompressible noise of both $X$ and $Y$ would make the analysis much more complex since they should not model neither the common nor the salient generative factors. We have empirically found that using only ($\bz$, $\bs$) gives already good results. 

%As in \cite{Goodfellow2014,chen_infogan_2016}, we introduce a generator $G$ and a discriminator $D$ that are trained together in a \textit{min-max} game. The generator $G$ should generate samples that are indistinguishable from the true ones whereas the discriminator $D$ is trained to discriminate between the fake and the real samples. 

%Let $X=G(\bz,0)$, $Y=G(\bz,\bs)$ the generated samples. As in InfoGAN, we make the hypothesis that the latent variables $\bz=\{z_1,z_2,...,z_L \}$ and $\bs=\{s_1, s_2, ..., s_M \}$ are independent and follow a factored distribution: $P(\bz)=\prod_{i=1}^L P(c_z)$ and $P(\bs)=\prod_{j=1}^M P(s_j)$. 

% \textit{Proof} $I(X;Y|z) = 0$: We first notice that $X$ only depends on $z$ and therefore $H(X|z)=0$. From this follows that $H(X|Y,z)=0$, since $H(X|Y,z) \geq 0$ and $H(X|Y,z) \leq H(X|z) = 0$. The mutual information between $X$ and $Y$, conditioned by the latent $c$, is then zero since $I(X;Y|z) = H(X|z)-H(X|Y,z) = 0$. This means that $Y$ is conditionally independent of $X$ given $z$.

%Similarly to InfoGAN, we add a regularization term based on mutual information between the generated samples and the latent codes. However, in our case this term is added not to disentangle between informative and nuisance generative factors but to \textit{separate} common and salient factors. We propose to maximize $I((z,s);y)$ and $I((z,s=s');x)$ as regularization terms. Their optimization force $\bz$ to fully encode alone $X$ since the salient factors $\bs$ of $X$ are forced to a constant value, here 0.

Since $\bz$ and $\bs$ are supposed to be independent, the mutual information $I((\bz,\bs); \by)$ can be decomposed into the sum of the two mutual information $I(\bz; \by) + I(\bs ; \by)$

\begin{equation}
\begin{split}
 &I((\bz, \bs);\by) = -H((\bz, \bs) | \by) + H(\bz , \bs) = -H((\bz, \bs) | \by) + H(\bz) + H(\bs)=\\
 &= \int \int \int P(\bz , \bs , \by) \log(\frac{P(\bz , \bs , \by)}{P(\by)}) dz ds dy + H(\bz) + H(\bs)=\\
 &= \int P(\by) \int \int P(\bs | \by) P(\bz|\by)  \log(P(\bs | \by) P(\bz|\by) ) dz ds dy + H(\bz) + H(\bs)= \quad \text{(suppose $P(\bs,\bz|\by)=P(\bs | \by) P(\bz|\by) )$}\\
 &= \int P(\by) \int \int P(\bs | \by) P(\bz|\by) \left( \log(P(\bs | \by)) + \log(P(\bz|\by) ) \right) dz ds dy + H(\bz) + H(\bs)=\\
 &= \int_y P(\by) \left ( \int_s P(\bs | \by) \log(P(\bs | \by)) + \int_z P(\bz|\by) \log(P(\bz|\by) )\right) dz ds dy + H(\bz) + H(\bs)=\\
 &=\bbE_{\by \sim P(\by), \bs \sim P(\bs | \by)} \log(P(\bs | \by) + \bbE_{\by \sim P(\by), \bz \sim P(\bz | \by)} \log(P(\bz | \by) + H(\bz) + H(\bs)=\\
 &= -H(\bs | \by) - H(\bz | \by) + H(\bz) + H(\bs) = I(\bz; \by) + I(\bs ; \by)
 \label{eq:DoubleInfoGAN}
\end{split}
\end{equation}

%Thus, similarly to InfoGAN (see Eq. \ref{app:InfoGAN-I} and Eq. \ref{app:InfoGAN-loss}), we can retrieve two lower bounds:

%\begin{equation}
%\begin{split}
% I(\bz;\by) &\geq  \bbE_{\bz \sim P(\bz), \bs \sim P(\bs),\by \sim P(\by |\bz, \bs)} \bbE_{\bz' \sim P(\bz'|\by)} \log( Q(\bz'|\by)) + H(\bz')\\
% &= \bbE_{\bz \sim P(\bz), \bs \sim P(\bs), \by \sim P(\by |\bz, \bs)} \log(Q(\bz|\by)) + H(\bz)
% \label{eq:lossZ}
%\end{split}
%\end{equation}

%\begin{equation}
%\begin{split}
% I(\bs;\by) &\geq  \bbE_{\bz \sim P(\bz), \bs \sim P(\bs),\by \sim P(\by |\bz, \bs)} \bbE_{\bs' \sim P(\bs'|\by)} \log( Q(\bs'|\by)) + H(\bs')\\
% &= \bbE_{\bz \sim P(\bz), \bs \sim P(\bs), \by \sim P(\by |\bz, \bs)} \log(Q(\bs|\by)) + H(\bs)
%  \label{eq:lossS}
%\end{split}
%\end{equation}

%Similarly to InfoGAN, to promote stability and efficiency, we propose to use a factorized distribution for the conditional distribution $q$. In addition to a factorized Gaussian distribution with identity covariance, we have also tested a factorized Laplace distribution $\bL(\mu,b)$ with $b=1$. This brings to a $l1$ reconstruction loss instead of a standard $l2$, and shows better performance in practice.

%When computing $I((\bz, \bs=s');\bx)$, the main difference lies in the definition of $P(\bs)$. Indeed, we choose the same factorized prior distribution $P(\bz)$ for both $X$ and $Y$, namely a Gaussian $\cN(0,1)$ or uniform distribution $\cU_{[-1,1]}$. However, for $P(\bs)$, we use a factorized uniform distribution $\cU_{(0,1]}$ for $Y$ and a Dirac delta distribution centered at 0 $\delta(\bs = 0)$ for $X$. In this way, we force the salient distribution $P(\bs)$ to be 0 for samples in $X$ and different from 0 for samples in $Y$. Please note that in practice we have also tested a factorized Gaussian $\cN(0,1)$ or uniform $\cU_{[-1,1]}$ distribution for $Y$ (ignoring the samples equal to 0) and results were very similar. 

%To better train the auxiliary distribution $q$, and since we know that $\bs$ should be equal for images in the $X$ domain, we also add as regularization the mutual information $I(\bs;\bx_R)$, where $\bx_R \sim P(\bx_R)$ are the actual training images. Similarly to Eq.\ref{eq:lossS}, we can derive a lower bound:

%\begin{equation}
 %I(\bs;\bx_R) \geq  \bbE_{\bx_R, \bs \sim P(\bx_R, \bs)} \log( Q(\bs|\bx_R)) + H(\bs) = \bbE_{\bx_R \sim P(\bx_R), \bs \sim P(\bs)} \log( Q(\bs|\bx_R)) + H(\bs)
%\label{eq:lossS-R}
%\end{equation}

%since the actual images $\bx_R$ do not depend on $\bs$. As before, we fix $P(\bs) = \delta(\bs = 0)$.

%Finally, another new loss is the log-likelihood $\log(P(x))$ of the generated images based on the proposed model. Indeed, no likelihood is generally available for optimizing the generator $G$ in a GAN model \cite{Goodfellow2014}. However, here, given a real image $\bx_R$ (or $\by_R$), we can use the auxiliary network $q$ to estimate the latent factors $\hat{z}$ and $\hat{s}$ that should generate $\bx_R$ (or $\by_R$) and then maximize (an approximation) of the log-likelihood of the generated images $x=G(\hat{z},0)$ (or $y=G(\hat{z},\hat{s})$). 
The log-likelihood $\log(P(y))$ of the generated images based on the proposed model is:

\begin{equation}
\begin{split}
 &\log P(\by) = \log \int \int \int P(\by,\bz,\bs,\by_R) dz ds dy_R = \log \int \int \int P(\by|\bz,\bs,\by_R) P(\bz,\bs|\by_R) P(\by_R) \frac{Q(\bz,\bs|\by_R)}{Q(\bz,\bs|\by_R)} dz ds dy_R\\
 &= \log \bbE_{\by_R \sim P(\by_R), (\bz,\bs) \sim Q(\bz, \bs |\by_R)} P(\by|\bz,\bs,\by_R)\frac{P(\bz,\bs|\by_R)}{Q(\bz,\bs|\by_R)} \geq \bbE_{\by_R \sim P(\by_R), (\bz,\bs) \sim Q(\bz, \bs |\by_R)} \log P(\by|\bz,\bs,\by_R)\frac{P(\bz,\bs|\by_R)}{Q(\bz,\bs|\by_R)}=\\
 &= \bbE_{\by_R \sim P(\by_R), (\bz,\bs) \sim Q(\bz, \bs |\by_R)} \log P(\by|\bz,\bs,\by_R) - \bbE_{\by_R \sim P(\by_R)} KL(Q(\bz,\bs|\by_R) || P(\bz,\bs|\by_R))
\end{split}
\end{equation}

%We can notice that the second term is always negative and it should tend towards 0 during training thanks to the previous Info Loss. We can thus approximate $\log P(\by)$ computing only the left term, namely $\bbE_{\by_R \sim P(\by_R), (\bz,\bs) \sim Q(\bz, \bs |\by_R)} \log P(\by|\bz,\bs,\by_R)$, and modeling $P(\by|\bz,\bs,\by_R)$ as a Laplace distribution $\bL(\mu,b)$ with $y=G(\hat{z},\hat{s})$, $\mu=\by_R$ and $b=1$. We use a Laplace distribution, instead of a Gaussian distribution, since it has been shown, for instance in \cite{isola_image--image_2017}, that a $l1$-loss encourages sharper and better image reconstructions than a $l2$-loss.

%\section{Wyner's common information}
%The common information between two random variables $X$ and $Y$, based on Wyner's principle \cite{wyner_common_1975}, is given by a third random variable $Z$ such that $X$ and $Y$ are conditionally independent given $Z$, but at the same time $Z$ should be as compact as possible.  Wyner proposed in \cite{wyner_common_1975} to measure compactness as the mutual information that $Z$ retains about $X$ and $Y$. The resulting optimization problem is not a convex problem and thus difficult to solve in practice.

%\textbf{Definition} For random variables $X$ and $Y$ with joint distribution $P(x,y)$, Wyner's common information is defined as:

%\begin{equation}
%C(X;Y)=\min_{P(z|x,y)} I(X,Y;Z) \text{ such that } I(X;Y|Z)=0   
%\end{equation}

%In our case, we know that by construction $X$ only depends on $Z$ and therefore $H(X|Z)=0$. From this follows that $H(X|Y,Z)=0$, since $H(X|Y,Z) \geq 0$ and $H(X|Y,Z) \leq H(X|Z) = 0$. The mutual information between $X$ and $Y$, conditioned by the latent $Z$, is then zero since $I(X;Y|Z) = H(X|Z)-H(X|Y,Z) = 0$. This means that $Y$ is conditionally independent of $X$ given $Z$. This shows that the constraint $I(X;Y|Z)=0 $ is thus always satisfied in our problem. The remaining optimization problem can be rewritten as: $\min_{P(z|x,y)} I(X,Y;Z)$ = $H(Z) - H(Z | X,Y)$. Since $I(X,Y;Z) \geq 0$, we obtain the minimum at $H(Z) = H(Z | X,Y)$, which means, for instance, when $P(Z)=P(Z|X,Y)$. Minimize $KL(P(Z) || P(Z|X,Y))$ ? Another path is given by the fact that $H(Z | X,Y) \leq H(Z)$ and thus we want to maximize $H(Z | X,Y)$. Another path is using CLUB (\url{http://proceedings.mlr.press/v119/cheng20b/cheng20b.pdf}).


\section{Losses equations}\label{app:loss}

In this section, we detail the different losses used in our paper as functions of the involved modules: discriminator, generator, encoder.
%In the following we write these functions for the generator and the discriminator separately, so that the indicated functions are to be minimized. 
Notation are as follows : from an image $I$, $D(I)$ will be the standard adversarial output of the GAN discriminator (namely the probability that an image is real or fake), $C(I)$ will be the class predicted by the discriminator from image $I$, and $Q(I)$ will be the predicted $\hat{z}$ and $\hat{s}$. In practice, Q, C and D share most of the layers (see detailed architecture). 

Reminder of the global loss : 

\begin{equation}
\label{eq:cr}
\begin{split}
    \underset{G,Q,H,C}{min} \underset{D}{max} \quad w_{Adv}  \cdot \mathcal{L}_{Adv}(G,D) +  w_{Class} \cdot \mathcal{L}_{Class}(G,C) \\ 
    + w_{Info}  \cdot \mathcal{L}_{Info}(G,Q) 
    + w_{Im} \cdot \mathcal{L}_{Im}(G,Q) \\
    + w_{CR}  \cdot \mathcal{L}_{CR}(G,H)
\end{split}
\end{equation}


\subsection{Adversarial GAN Loss}\label{app:eq-Adv}
Similarly to \cite{Goodfellow2014}, the adversarial loss used here is: 
\begin{equation}
\begin{split}
    \mathcal{L}_{Adv}(D,G) = w_{bg}  \Bigl( - \mathbb{E}_{\bx_R\sim P(\bx_R)}\bigl[\log(D(\bx_R)\bigr] - 
    \mathbb{E}_{z \sim P_x(\bz)}\bigl[\log(1-(D(G(\bz,0))))\bigr] \Bigr) \\
    w_t \Bigl( - \mathbb{E}_{\by_R\sim P(\by_R)}\bigl[\log(D(\by_R)\bigr] 
    - \mathbb{E}_{\bz,\bs \sim P_y(\bz,\bs)}\bigl[\log(1-(D(G(\bz,\bs))))\bigr]\Bigr)
\end{split}
\end{equation}

%\begin{equation}
%    \mathcal{L}_{NSGAN}^G = - w_{bg}\cdot\mathbb{E}_{z\sim \mathcal{N}(0,1)}%[\log(D(G(z,0))] - w_t \cdot \mathbb{E}_{z,s\sim \mathcal{N}(0,1)}[\log(D(G(z,s))] 
%\end{equation}

%\subsection{Class Loss}


%Labels for class X (resp. Y) are arbitrarily 0 (resp. 1). We use the binary cross entropy (BCE). The discriminator $C$ is trained on real images only to distinguish background images X from target images Y, and the generator is trained using the output of C. The generator is trained so that the images $G(z,0)$ are labeled 0, as the images of the background X, and that the images $G(z,s)$ are labeled 1, as the target images of Y.

%\begin{equation}
%    \mathcal{L}_{class}^{C} = w_{bg} \mathbb{E}_{\bx_R\sim P(\bx_R)}\bigl[BCE(C(\bx_R), 0)\bigr] +  w_t  \mathbb{E}_{\by_R\sim P(\by_R)}\bigl[BCE(C(\by_R), 1)\bigr]
%\end{equation}


%\begin{equation}
%    \mathcal{L}_{Class}^G = w_{bg} \mathbb{E}_{z\sim \mathcal{N}(0,1)}[BCE(C(G(z,0)), 1)] + w_t \cdot \mathbb{E}_{z,s \sim \mathcal{N}(0,1)}[BCE(C(G(z,s)), 0)]
%\end{equation}



\subsection{Info Loss}

%The info loss is the same for the generator G and the output Q of the discriminator, the goal being always to reconstruct z and s, similarly to InfoGAN. However, here we have also added another term for Q.  When a real background image $I_X$ is used, we also want $Q_s(I_X)$ to be zero. 
The weight $w_{Info}$ is actually divided in three components : $w_{Info}^s$, $w_{Info}^z$ and $w_{Info}^{real}$

\begin{equation}
\begin{split}
    \mathcal{L}_{Info}(G,Q) &= w_{bg} \mathbb{E}_{\bz \sim P_y(\bz)}\bigl[w_{Info}^z |(Q_z(G(z,0))- z| + w_{Info}^s |Q_s(G(z,0))- 0|\bigr]\\
    &+ w_t \mathbb{E}_{\bz,\bs \sim P_y(\bz,\bs)}\bigl[w_{Info}^z  |(Q_z(G(z,s))- z| + w_{Info}^s |Q_s(G(z,s))- s|\bigr]\\& +  w_{Info}^{real} \mathbb{E}_{\bx_R \sim P(\bx_R)}\bigl[|(Q_s(\bx_R))- 0|\bigr]
\end{split}
\end{equation}


\subsection{Image reconstruction loss}
We also use an image reconstruction loss, which depends on G and Q: 

\begin{equation}
    \mathcal{L}_{Im}(G,Q) = w_{bg} \mathbb{E}_{ \bx_R \sim P(\bx_R), \hat{z}=Q_z(\bx_R)}\bigl[|G(\hat{z},0) - \bx_R|\bigr] +  w_t \mathbb{E}_{\by_R \sim P(\by_R), \hat{z}, \hat{s}=Q(\by_R)}\bigl[|G(\hat{z},\hat{s}) - \by_R|\bigr]
\end{equation}


\subsection{CR Loss}\label{app:CR-loss}

The Contrastive Regularization loss is computed to improve the disentanglement of $\bs$. The module H and the generator G are trained using a Cross Entropy loss to find the salient feature $k$ in common between two images generated with two salient factors that have only one factor in common (i.e., $s^1_k = s^2_k$) and all other factors different (i.e., $s^1_j \neq s^2_j$ with $\forall j \neq k$):

\begin{equation}
    \mathcal{L}_{CR}(G,H) = \mathbb{E}_{k \in \mathbb{N}, z \sim P_y(\bz), s^1,s^2 \sim P_y(\bs), s^1_k = s^2_k, s^1_j \neq s^2_j, \forall j \neq k}\Bigl[CE\bigl(H(G(z,s^1), G(z,s^2)), k\bigr)\Bigr]
\end{equation}


\subsection{Weights and ratio between the losses}
Different weights are used to balance the different losses, as well as other hyper-parameters (learning rate, number of epochs, etc.). Table~\ref{tab:weights} summarizes the hyper-parameters used in our experiments and their values for each dataset employed. %for the purpose of reproducibility

\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
 \multirow{2}{*}{parameters}  &  \multirow{2}{*}{definition} &  \multicolumn{4}{c}{value for different datasets} \\
&  & celeba & cifar-mnist  & mnist-dsprite & brats\\
\hline
loop G  & number of G loop & 1 & 1 & 2 & 1 \\
loop D  & number of D loop & 1 & 1 & 1 & 1 \\
loop CR (when used) & number of CR loop & - & 1 & 1 & 1 \\
lr G    & learning rate G & 0.0002 & 0.0002 & $5\cdot 10^{-5}$ & 0.0001\\
lr D    & learning rate D & 0.0002 & 0.0002 & $5\cdot 10^{-5}$ & 0.0001\\
lr CR  (when used) & learning rate CR & - & 0.0002 & $5\cdot 10^{-5}$ & 0.0001\\
$w_{bg}$& weight for background & 0.5 & 0.5 & 0.5 & 0.5\\
$w_t$   & weight for target losses & 1.0 & 1.0 & 1.0 & 1.0\\
$w_{Adv}$ & weight for adversarial loss & 0.5 & 0.5 & 0.5 & 0.5\\
$w_{Class}$ & weight for class classification & 0.5 & 0.5 & 0.5 & 0.5\\
$w_{Image}$ & weight for image reconstruction & 1.0 & 1.0 & 1.0 & 1.0\\
$w_{Info}^z$ & weight for info loss z & 1.0 & 1.0 & 1.0 & 1.0\\
$w_{Info}^s$ & weight for info loss s & 1.0 & 1.0 & 1.0 & 1.0 \\
$w_{Info}^{real}$ & weight for info loss real image & 1.0 & 1.0 & 1.0 & 1.0 \\
$w_{CR}$ (when used) & weight for CR loss & - & 1.0 & 1.0 & 1.0\\
    \end{tabular}
    \caption{Hyperparameters used for every dataset}
    \label{tab:weights}
\end{table}


\section{Extensive Results}\label{app:extensive-results}

\begin{table}
    \centering
    \begin{tabular}{c|c c | c c }
    original images &  \multicolumn{2}{c|}{Image reconstruction}  &  \multicolumn{2}{c}{Image swap} \\
                        & MM-cVAE & double InfoGAN & MM-cVAE & double InfoGAN \\
        \includegraphics[width=2cm]{figures/bg5.png} & \includegraphics[width=2cm]{figures/recon_bg_mmcvae5.png} & \includegraphics[width=2cm]{figures/recon_bg_infogan5.png} & \includegraphics[width=2cm]{figures/swap_bg_mmcvae5.png} & \includegraphics[width=2cm]{figures/swap_bg_infogan5.png} \\
        \includegraphics[width=2cm]{figures/target5.png} & \includegraphics[width=2cm]{figures/recon_t_mmcvae5.png} & \includegraphics[width=2cm]{figures/recon_t_infogan5.png} & \includegraphics[width=2cm]{figures/swap_t_mmcvae5.png} & \includegraphics[width=2cm]{figures/swap_t_infogan5.png} \\
        \hline \\
        \includegraphics[width=2cm]{figures/bg11.png} & \includegraphics[width=2cm]{figures/recon_bg_mmcvae11.png} & \includegraphics[width=2cm]{figures/recon_bg_infogan11.png} & \includegraphics[width=2cm]{figures/swap_bg_mmcvae11.png} & \includegraphics[width=2cm]{figures/swap_bg_infogan11.png} \\
        \includegraphics[width=2cm]{figures/target11.png} & \includegraphics[width=2cm]{figures/recon_t_mmcvae11.png} & \includegraphics[width=2cm]{figures/recon_t_infogan11.png} & \includegraphics[width=2cm]{figures/swap_t_mmcvae11.png} & \includegraphics[width=2cm]{figures/swap_t_infogan11.png} \\
        \hline \\
        \includegraphics[width=2cm]{figures/bg56.png} & \includegraphics[width=2cm]{figures/recon_bg_mmcvae56.png} & \includegraphics[width=2cm]{figures/recon_bg_infogan56.png} & \includegraphics[width=2cm]{figures/swap_bg_mmcvae56.png} & \includegraphics[width=2cm]{figures/swap_bg_infogan56.png} \\
        \includegraphics[width=2cm]{figures/target56.png} & \includegraphics[width=2cm]{figures/recon_t_mmcvae56.png} & \includegraphics[width=2cm]{figures/recon_t_infogan56.png} & \includegraphics[width=2cm]{figures/swap_t_mmcvae56.png} & \includegraphics[width=2cm]{figures/swap_t_infogan56.png} \\
    \end{tabular}
    \captionof{figure}{Image reconstruction and swap with CelebA. In every block, first row refers to $X$ and second row to $Y$. It's interesting to notice that rare attributes, such as the glasses in the first two blocks, are correctly reconstructed by our method and not by MM-cVAE. However, they are changed towards  more "common" glasses after swapping.}
    \label{tab:my_label}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{|c |cc |cc |cc  | c c |c c |} 
\hline
&  \multicolumn{10}{|c|}{cVAE}   \\ 
& \multicolumn{2}{c|}{epoch 100}   & \multicolumn{2}{c|}{epoch 200} & \multicolumn{2}{c|}{epoch 300} & \multicolumn{2}{c|}{epoch 400} & \multicolumn{2}{c|}{epoch 500} \\
& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ \\

Training 1  & $0.81$ & $0.80$ & $0.82$ & $0.80$ & $0.83$ & $0.80$ & $0.82$ & $0.79$ & $0.83$ & $0.80$  \\
Training 2  & $0.78$ & $0.82$ & $0.80$ & $0.82$ & $0.79$ & $0.82$ & $0.80$ & $0.81$ & $0.81$ & $0.81$ \\
Training 3  & $0.79$ & $0.82$ & $0.79$ & $0.82$ & $0.80$ & $0.81$ & $0.81$ & $0.81$ & $0.81$ & $0.81$ \\
Training 4 & $0.83$ & $0.79$ & $0.84$ & $0.78$ & $0.83$ & $0.78$ & $0.84$ & $0.78$ & $\mathbf{0.84}$ & $\mathbf{0.78}$ \\
Training 5 & $0.79$ & $0.82$ & $0.80$ & $0.81$ & $0.82$ & $0.81$ & $0.81$ & $0.80$ & $0.82$ & $0.80$ \\
 \hline
&  \multicolumn{10}{|c|}{MM-cVAE}   \\ 
& \multicolumn{2}{c|}{epoch 100}   & \multicolumn{2}{c|}{epoch 200} & \multicolumn{2}{c|}{epoch 300} & \multicolumn{2}{c|}{epoch 400} & \multicolumn{2}{c|}{epoch 500} \\
& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ \\

Training 1 & $0.84 $ & $0.75 $ & $0.84 $ & $0.75$ & $0.85 $ & $0.73$ & $0.85$ & $0.73 $ & $\mathbf{0.85}$ & $\mathbf{0.72}$ \\
Training 2 & $0.83$ & $0.77$ & $0.84$ & $0.76$ & $0.85$ & $0.75$ & $0.85$ &$0.75$ & $0.85$ & $0.74$ \\ 
Training 3 & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ \\
Training 4 &$0.79$& $0.82$ & $0.80$& $0.83$ & $0.73$ & $0.83$ & $0.74$ & $0.83$ & $0.74 $ & $0.83 $ \\
Training 5 & $0.81$ & $0.79$ & $0.82$ & $0.79$ & $0.82$ & $0.79$ & $0.83$ & $0.78$ & $0.83 $ & $0.77 $ \\

 \hline

 &  \multicolumn{10}{|c|}{double InfoGAN}  \\
%  & \multicolumn{2}{c|}{epoch 100}   & \multicolumn{2}{c|}{epoch 200} & \multicolumn{2}{c|}{epoch 300} & \multicolumn{2}{c|}{epoch 400} & \multicolumn{2}{c|}{epoch 500} \\
% & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ \\

% Training 1 & $0.87$ & $0.78$ & $0.90$ & $0.73$ & $0.92$ & $0.73$ & $0.93$ & $0.74$ & $0.93 $ & $0.72 $\\
% Training 2 & $0.87$ & $0.80$ & $0.89$ & $0.77$ & $0.90$ & $0.73$ & $0.91$ & $0.77$ &  $0.92 $ & $0.72$ \\
% Training 3 & $0.89$ & $0.84$ & $0.90$ & $0.74$ & $0.91$ & $0.74$ & $0.93$ & $0.74$ &  $0.93 $ & $0.72 $ \\
% Training 4 & $0.85$ & $0.82$ & $0.89$ & $0.75$ & $0.91$ & $0.74$ & $0.92$ & $0.73$ & $\mathbf{0.93}$ & $\mathbf{0.71}$ \\
% Training 5 & $0.78$ & $0.80$ & $0.78$ & $0.81$ & $0.79$ & $0.80$ & $0.81$ & $0.81$ & $0.83$ & $0.79$ \\
% \hline
%  &  \multicolumn{10}{|c|}{double InfoGAN (no CR)}  \\
 & \multicolumn{2}{c|}{epoch 100}   & \multicolumn{2}{c|}{epoch 200} & \multicolumn{2}{c|}{epoch 300} & \multicolumn{2}{c|}{epoch 400} & \multicolumn{2}{c|}{epoch 500} \\

 
& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$ & $s_x$ $\uparrow$ & $z_x$ $\downarrow$& $s_x$ $\uparrow$ & $z_x$ $\downarrow$ \\

Training 1 & $0.93$ & $0.74$ & $0.93$ & $0.73$ & $0.95$ & $0.72$ & $0.95$ & $0.73$ & $0.94$ & $0.70$\\
Training 2 & $0.92$ & $0.70$ & $0.94$ & $0.73$ & $0.95$ & $0.73$ & $0.95$ & $0.74$ & $0.95$ & $0.73$\\
Training 3 & $0.92$ & $0.69$ & $0.94$ & $0.71$ & $0.95$ & $0.74$ & $0.95$ & $0.73$ & $\mathbf{0.95}$ & $\mathbf{0.69}$\\
Training 4 & $0.93$ & $0.72$ & $0.94$ & $0.70$ & $0.95$ & $0.72$ & $0.95$ & $0.71$ & $0.95$ & $0.72$ \\
Training 5 & $0.93$ & $0.72$ & $0.94$ & $0.70$ & $0.95$ & $0.72$ & $0.95$ & $0.76$ & $0.95$ & $0.73$ \\
\hline
\end{tabular}
\end{center}
\caption{Target Dataset separation on CelebA - glasses vs hat - for the 5 trainings of the three methods at different epochs. For clarity, we don't report the standard deviations, whose values are between 0.00 and 0.01. We can notice that the trainings of MMc-VAE are less stable than the ones of our method.}
\label{tab:target-sep-celeba2}
\end{table}


\begin{table}
\begin{center}
\begin{tabular}{|c |cccc |cccc  |cccc|} 
\hline
 &  \multicolumn{12}{|c|}{MM-cVAE with latent space size $128$ $(64\times 2)$}  \\
 
 & \multicolumn{4}{c|}{epoch 100}   & \multicolumn{4}{c|}{epoch 300} & \multicolumn{4}{c|}{epoch 500} \\
 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)}\\
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ \\ 
 
Training 1  & $0.68$ & $0.57$ & $0.16$ & $0.36$ & $0.68$ & $0.51$ & $0.15$ & $0.36$ & $0.70$ & $0.49$ & $0.16$ & $0.36$ \\
Training 2  & $0.80$ & $0.51$ & $0.15$ & $0.36$ & $0.80$ & $0.41$ & $0.16$ & $0.36$ & $\mathbf{0.81}$ & $\mathbf{0.43}$ & $\mathbf{0.14}$ & $\mathbf{0.36}$  \\
Training 3  & $0.81$ & $0.56$ & $0.27$ & $0.33$ & $0.81$ & $0.52$ & $0.27$ & $0.33$ & $0.81$ & $0.52$ & $0.27$ & $0.33$ \\
Training 4  & $0.81$ & $0.53$ & $0.31$ & $0.25$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ & $nan$ \\
Training 5  & $0.71$ & $0.57$ & $0.16$ & $0.35$ & $0.73$ & $0.51$ & $0.15$ & $0.36$ & $0.74$ & $0.47$ & $0.16$ & $0.36$ \\
\hline
 &  \multicolumn{12}{|c|}{MM-cVAE with latent space size $200$ $(100\times 2)$}  \\
 
 & \multicolumn{4}{c|}{epoch 100}   & \multicolumn{4}{c|}{epoch 300} & \multicolumn{4}{c|}{epoch 500} \\
 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)}\\
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ \\ 

Training 1  & 0.19 & 0.82 & 0.12 & 0.35 & 0.14 & 0.82 & 0.12 & 0.36 & 0.13 & 0.82 & 0.12 & 0.35 \\
Training 2  & 0.80 & 0.55 & 0.17 & 0.36 & 0.80 & 0.44 & 0.16 & 0.37 & 0.80 & 0.43 & 0.16 & 0.37  \\
Training 3  & 0.81 & 0.64 & 0.28 & 0.34 & 0.82 & 0.57 & 0.27 & 0.34 & 0.82 & 0.55 & 0.27 & 0.34 \\
Training 4  & 0.66 & 0.67 & 0.18 & 0.36 & 0.64 & 0.63 & 0.16 & 0.36 & 0.61 & 0.60 & 0.15 & 0.36 \\
Training 5  & 0.76 & 0.60 & 0.19 & 0.36 & 0.78 & 0.51 & 0.17 & 0.37 & 0.79 & 0.48 & 0.17 & 0.37 \\
\hline
 &  \multicolumn{12}{|c|}{double InfoGAN with latent space size $200$ $(100\times 2)$}  \\
 
 & \multicolumn{4}{c|}{epoch 100}   & \multicolumn{4}{c|}{epoch 300} & \multicolumn{4}{c|}{epoch 500} \\
 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)}\\
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ \\ 

Training 1  & 0.89 & 0.28 & 0.19 & 0.42 & 0.89 & 0.30 & 0.20 & 0.44 & 0.88 & 0.32 & 0.20 & 0.44\\
Training 2  & 0.89 & 0.29 & 0.21 & 0.41 & 0.88 & 0.31 & 0.22 & 0.43 & 0.87 & 0.32 & 0.22 & 0.44  \\
Training 3  & 0.90 & 0.28 & 0.19 & 0.42 & 0.88 & 0.32 & 0.21 & 0.44 & 0.88 & 0.32 & 0.21 & 0.44 \\
Training 4  & 0.90 & 0.29 & 0.20 & 0.41 & 0.88 & 0.30 & 0.22 & 0.43 & 0.86 & 0.32 & 0.23 & 0.43 \\
Training 5  & 0.89 & 0.28 & 0.19 & 0.41 & 0.88 & 0.30 & 0.21 & 0.44 & 0.86 & 0.32 & 0.22 & 0.43 \\
\hline
 &  \multicolumn{12}{|c|}{double InfoGAN with latent space size $128$ $(64\times 2)$ }  \\
 
 & \multicolumn{4}{c|}{epoch 100}   & \multicolumn{4}{c|}{epoch 300} & \multicolumn{4}{c|}{epoch 500} \\
 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)}\\
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ \\ 

Training 1  & 0.88 & 0.21 & 0.16 & 0.40 & 0.88 & 0.27 & 0.18 & 0.42 & $\mathbf{0.87}$ & $\mathbf{0.26}$ & $\mathbf{0.18}$ & $\mathbf{0.43}$ \\
Training 2  & 0.87 & 0.24 & 0.16 & 0.39 & 0.88 & 0.27 & 0.16 & 0.43 & 0.87 & 0.26 & 0.17 & 0.43  \\
Training 3  & 0.88 & 0.22 & 0.16 & 0.39 & 0.87 & 0.26 & 0.18 & 0.42 & 0.86 & 0.26 & 0.19 & 0.42\\
Training 4  & 0.87 & 0.25 & 0.17 & 0.40 & 0.88 & 0.25 & 0.19 & 0.42 & 0.87 & 0.28 & 0.19 & 0.41 \\
Training 5  & 0.88 & 0.24 & 0.15 & 0.39 & 0.87 & 0.24 & 0.17 & 0.42 & 0.86 & 0.25 & 0.19 & 0.43 \\
\hline
 &  \multicolumn{12}{|c|}{double InfoGAN with latent space size $128$ $(64\times 2)$ with CR module}  \\
 
 & \multicolumn{4}{c|}{epoch 100}   & \multicolumn{4}{c|}{epoch 300} & \multicolumn{4}{c|}{epoch 500} \\
 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
 & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)}\\
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
 & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ \\ 

Training 1  & $0.88$ & $0.25$ & $0.18$ & $0.42$ & $0.87$ & $0.28$ & $0.18$ & $0.43$ & $0.87$ & $0.26$ & $0.18$ & $0.43$ \\
Training 2  & $0.87$ & $0.23$ & $0.16$ & $0.40$ & $0.88$ & $0.24$ & $0.18$ & $0.43$ & $0.87$ & $0.26$ & $0.18$ & $0.42$  \\
Training 3  & $0.88$ & $0.21$ & $0.18$ & $0.40$ & $0.88$ & $0.26$ & $0.19$ & $0.43$ & $0.87$ & $0.28$ & $0.20$ & $0.43$ \\
Training 4  & $0.88$ & $0.26$ & $0.17$ & $0.39$ & $0.88$ & $0.27$ & $0.18$ & $0.42$ & $0.88$ & $0.26$ & $0.19$ & $0.42$ \\
Training 5  & $0.89$ & $0.26$ & $0.17$ & $0.40$ & $0.88$ & $0.25$ & $0.18$ & $0.42$ & $\mathbf{0.87}$ & $\mathbf{0.26}$ & $\mathbf{0.18}$ & $\mathbf{0.43}$ \\
\hline
\end{tabular}
\end{center}
\caption{Target Dataset separation on Cifar-10-MNIST for MM-cVAE and our method, with and without CR module, and for different latent space sizes. We report the results of the 5 trainings per method at different epochs. For clarity, we don't report the standard deviations, whose values are between 0.00 and 0.01. Even here, the trainings of MMc-VAE are less stable than the ones of our method, regardless of the latent dimension.}
\label{tab:target-sep-cifar2}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{c|c c | c c }
    Original &  \multicolumn{2}{c}{Reconstruction}  & \multicolumn{2}{c}{Swap} \\
                        & MM-  & double & MM- & double  \\
                        & cVAE &  InfoGAN & cVAE & InfoGAN \\
        \includegraphics[width=1.7cm]{figures/cifar_bg21.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_mmcvae21.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_infogan21.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_mmcvae21.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_infogan21.png} \\
        \includegraphics[width=1.7cm]{figures/cifar_target21.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_mmcvae21.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_infogan21.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_mmcvae21.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_infogan21.png} \\
        \hline \\
        \includegraphics[width=1.7cm]{figures/cifar_bg14.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_mmcvae14.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_infogan14.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_mmcvae14.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_infogan14.png} \\
        \includegraphics[width=1.7cm]{figures/cifar_target14.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_mmcvae14.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_infogan14.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_mmcvae14.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_infogan14.png} \\
        \hline \\
        \includegraphics[width=1.7cm]{figures/cifar_bg27.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_mmcvae27.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_infogan27.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_mmcvae27.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_infogan27.png} \\
        \includegraphics[width=1.7cm]{figures/cifar_target27.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_mmcvae27.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_infogan27.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_mmcvae27.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_infogan27.png} \\
        \hline \\
        \includegraphics[width=1.7cm]{figures/cifar_bg61.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_mmcvae61.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_bg_infogan61.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_mmcvae61.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_bg_infogan61.png} \\
        \includegraphics[width=1.7cm]{figures/cifar_target61.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_mmcvae61.png} & \includegraphics[width=1.7cm]{figures/cifar_recon_t_infogan61.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_mmcvae61.png} & \includegraphics[width=1.7cm]{figures/cifar_swap_t_infogan61.png} \\
    \end{tabular}
    \captionof{figure}{More examples of image reconstruction and swap with Cifar-10-MNIST dataset.}
    \label{tab:cifar-img2}
\end{table}


% \begin{table}[h]
%     \centering
%     %\hspace{-0.3cm}
%     \begin{tabular}{|c|c c | c c }
%     Original &  \multicolumn{2}{c}{Reconstruction}  & \multicolumn{2}{c}{Swap} \\
%                         & MM-  & double & MM- & double  \\
%                         & cVAE &  InfoGAN & cVAE & InfoGAN \\
%         \includegraphics[width=2.0cm]{figures/dsprite_bg11.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_mmcvae11.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_infogan11.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_mmcvae11.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_infogan11.png} \\
%         \includegraphics[width=2.0cm]{figures/dsprite_target11.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_mmcvae11.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_infogan11.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_mmcvae11.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_infogan11.png} \\
%         \hline \\
%         \includegraphics[width=2.0cm]{figures/dsprite_bg46.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_mmcvae46.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_infogan46.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_mmcvae14.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_infogan46.png} \\
%         \includegraphics[width=2.0cm]{figures/dsprite_target46.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_mmcvae46.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_infogan46.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_mmcvae46.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_infogan46.png} \\
%         \hline \\
%         \includegraphics[width=2.0cm]{figures/dsprite_bg16.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_mmcvae16.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_infogan16.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_mmcvae16.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_infogan16.png} \\
%         \includegraphics[width=2.0cm]{figures/dsprite_target50.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_mmcvae16.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_infogan16.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_mmcvae16.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_infogan16.png} \\
%         \hline
%         \includegraphics[width=2.0cm]{figures/dsprite_bg14.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_mmcvae14.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_infogan14.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_mmcvae14.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_infogan14.png} \\
%         \includegraphics[width=2.0cm]{figures/dsprite_target14.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_mmcvae14.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_infogan14.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_mmcvae14.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_infogan14.png} \\
%         \hline \\
%         \includegraphics[width=2.0cm]{figures/dsprite_bg50.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_mmcvae50.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_bg_infogan50.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_mmcvae50.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_bg_infogan50.png} \\
%         \includegraphics[width=2.0cm]{figures/dsprite_target50.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_mmcvae50.png} & \includegraphics[width=2.0cm]{figures/dsprite_recon_t_infogan50.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_mmcvae50.png} & \includegraphics[width=2.0cm]{figures/dsprite_swap_t_infogan50.png} \\
%     \end{tabular}
%     \caption{Failure examples of image reconstruction and swap with dSprites-MNIST dataset.}
%     \label{tab:my_label}
% \end{table}



% \begin{table}[H]
% \begin{center}
% \begin{tabular}{|c |cccc |cccc  |cccc|} 
% \hline
%  &  \multicolumn{12}{|c|}{Ablation study on the losses}  \\
 
%  & \multicolumn{4}{c|}{epoch 100}   & \multicolumn{4}{c|}{epoch 300} & \multicolumn{4}{c|}{epoch 500} \\
 
%  & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
%  & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)} 
%  & \multicolumn{2}{c|}{Mnist (salient)} & \multicolumn{2}{c|}{Cifar (bg)}\\
%  & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
%  & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ 
%  & $s_y$ $\uparrow$ & $z_y$ $\downarrow$  & $s_y$ $\downarrow$ & $z_y$ $\uparrow$ \\ 
%  -$L_{Class}$ & 0.46 & 0.82 & 0.21 & 0.36 &	0.52 & 0.83 & 0.23 & 0.37 & 0.48 & 0.83 & 0.23 & 0.37 \\												
% - $L_{Class}$ - $L_{Im}$	& 0.44 & 0.8 & 0.22 & 0.36 & 0.48 & 0.79 & 0.23 & 0.38 & 0.54 & 0.72 & 0.22 & 0.38 \\	
% - $L_{Info}$ - $L_{Class}$ - $L_{Im}$ & 0.76 & 0.76 & 0.25 & 0.27 & 0.71 & 0.72 & 0.19 & 0.2 & 0.70 &	0.70 &	 0.18 & 0.18 \\						
% - $L_{Info}$ & 0.87 & 0.65 & 0.31 & 0.38 & 0.85 & 0.61 & 0.31 & 0.38 & 0.85 & 0.60 & 0.30 & 0.36 \\													
% - $L_{Info}^z$ & 0.85 & 0.77 & 0.36 & 0.36 & 0.86 & 0.74 & 0.39 & 0.35 & 0.86 & 0.743 & 0.387 & 0.347 \\												
% - $L_{Info}^s$ & 0.91 & 0.27 & 0.24 & 0.39 & 0.9 & 0.28 & 0.23 & 0.42 & \textbf{0.90} & \textbf{0.27} & 0.22 &  \textbf{0.43} \\
% - $L_{Info}^{s\_real_I}$	 & 0.88 & 0.24 & 0.17 & 0.40 & 0.87 & 0.3 & 0.18 & 0.42 &  \textbf{0.87} & \textbf{0.26} & \textbf{0.19} & \textbf{0.43} \\
% - $L_{Info}^s$ - $L_{Info}^{s\_real_I}$ & 0.87 & 0.28 & 0.32 & 0.40 & 0.85 & 0.26 & 0.30 & 0.43 & 0.83 & 0.27 & 0.30 & \textbf{0.44} \\
% - $L_{Info}$ - $L_{Im}$ & 0.74 & 0.72 & 0.25 & 0.26 & 0.62 & 0.62 & 0.21 & 0.22 & 0.59 & 0.59 & 0.20 & 0.20 \\
% - $L_{Class}$ - $L_{Info}$	& 0.79	& 0.75 & 0.32 & 0.36 & 0.75 & 0.68 & 0.3 & 0.35 & 0.74 & 0.67 & 0.29 & 0.35 \\
% - $L_{Im}$	& 0.87 & 0.24 & 0.18 & 0.40 & 0.87 & 0.25 & 0.19 & 0.42 & \textbf{0.86} & \textbf{0.25} &  \textbf{0.20} &  \textbf{0.43} \\
% Full & 0,88 & 0,24 & 0.16 & 0.39 & 0.87 & 0.25 & 0.18	& 0.42 & \textbf{0.87} & \textbf{0.26} &  \textbf{0.18} & \textbf{0.43} \\										
% \hline
% \end{tabular}
% \end{center}
% \caption{Ablation study of the different losses on cifar-MNIST dataset. For every configuration, 3 trainings were launched. Score indicated is the mean (standard deviation is below 0.01, so we don't report it for clarity)}
% \label{tab:ablation}
% \end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[width=14cm]{figures/RebuttalcVAE.png}
    \caption{Swap using the cVAE method with the
CelebA with accessories dataset. We can clearly see that personal traits (which should be encoded in the common space) are lost during the swap and accessories (which should be encoded in the salient space) are not always correctly added. This could explain the poor quantitative performance of cVAE.}
    \label{fig:rebuttal}
\end{figure}

\begin{table}
\begin{center}
\begin{tabular}{|c |c |c | c | c |c | c | c | c |} 
\hline
&  \multicolumn{8}{|c|}{With CR Loss}   \\ 
& epoch 50 & epoch 100 & epoch 200 & epoch 300 & epoch 400 & epoch 500 & epoch 600 & epoch 700 \\

Training 1 & 0.334 & 0.366 & 0.366 & 0.376 & 0.394 & 0.396 & 0.398& 0.4 \\
Training 2 & 0.414 & 0.37 & 0.338 & 0.328 & 0.314 & 0.314 & 0.282 & 0.294 \\	
Training 3 & 0.258 & 0.294 & 0.25 & 0.258 & 0.222 & 0.222 & 0.218 &	0.216 \\	
Training 4 & 0.35 & 0.346 & 0.346 & 0.402 & 0.43 & 0.454 & 0.49 & \textbf{0.494} \\	
Training 5 & 0.202 & 0.202 & 0.206 & 0.216 & 0.22 & 0.222 & 0.226 & 0.24 \\
 \hline
 
&  \multicolumn{8}{|c|}{No CR Loss}   \\ 
Training 1 & 0.348 & 0.358 & 0.364 & 0.376 & 0.39 & 0.392 & 0.406 &	\textbf{0.424} \\
Training 2 & 0.348 & 0.354 & 0.372 & 0.37 & 0.378 & 0.396 & 0.398 & 0.398 \\
Training 3 & 0.326 & 0.35 &	0.354 & 0.342 &	0.334 & 0.324 & 0.306 & 0.306 \\
Training 4 & 0.292 & 0.292 & 0.288 & 0.306 & 0.316 & 0.358 & 0.348 & 0.386 \\
Training 5 & 0.306 & 0.32 & 0.318 & 0.292 & 0.304 &	0.324 & 0.334 & 0.34 \\
\hline
\end{tabular}
\end{center}
\caption{Ablation study of CR Loss on Mnist-dsprite dataset. Score indicated is fvae score}
\label{tab:fvae}
\end{table}


